Quantum Algorithm Implementations for Beginners

As quantum computers become available to the general public, the need has arisen to train a cohort of quantum programmers, many of whom have been developing classical computer programs for most of their careers. While currently available quantum computers have less than 100 qubits, quantum computing hardware is widely expected to grow in terms of qubit count, quality, and connectivity. This review aims to explain the principles of quantum programming, which are quite different from classical programming, with straightforward algebra that makes understanding of the underlying fascinating quantum mechanical principles optional. We give an introduction to quantum computing algorithms and their implementation on real quantum hardware. We survey 20 different quantum algorithms, attempting to describe each in a succinct and self-contained fashion. We show how these algorithms can be implemented on IBM's quantum computer, and in each case, we discuss the results of the implementation with respect to differences between the simulator and the actual hardware runs. This article introduces computer scientists, physicists, and engineers to quantum algorithms and provides a blueprint for their implementations.

==> BV_Santhi/BV.tex <==
\newcommand{\V}[1]{\ensuremath{\mathbf #1}}

% Dirac Kets


\section{Bernstein-Vazirani Algorithm}
%\section{Bernstein-Vazirani Algorithm in IBM Quantum Experience}

\subsection{Problem definition and background}
Suppose we are given a classical Boolean function, $f : \{0,1\}^n \mapsto \{0,1\}$.
Such a function is guaranteed to be of the
 form, $f_\V{s}(\V{x}) = \braket{\V{s}, \V{x}}$.
Here, \V{s} is an unknown vector, which we shall call a \emph{hidden string}; and \braket{\cdot,\cdot} is the usual vector \emph{dot} product.
Let us also suppose that we are given a black-box implementation of this function, and are tasked with identifying the hidden string \V{s} with the least possible number of queries to the black box.

Since each classical query to this function produces just $1$ bit of information, and since an arbitrary hidden string \V{s} has $n$-bits of information, the classical \emph{query complexity} is seen to be $n$. Even with bounded error, there is no way that this classical complexity can be brought down, as can be seen using slightly more rigorous information theoretic arguments.

Bernstein and Vazirani~\cite{BV93} built upon the earlier work of Deutsch and Jozsa~\cite{DJ92} in theoretically exploring quantum query complexity. Their contribution to the field was a quantum algorithm for the hidden string problem, which has a non-recursive quantum query complexity of just $1$. This constitutes a polynomial $\mathcal{O}(n)$ query-complexity separation between classical and quantum computation. They also discovered a less widely known recursive hidden-string query algorithm, which shows a $\mathcal{O}(n^{\log{n}})$ separation between classical and quantum query-complexities. These developments preceded the more famous results of Shor and Grover, and kindled a lot of early academic interest in the inherent power of quantum computers.

One thing to note with respect to the Bernstein-Vazirani (BV) quantum hidden-string query algorithm is that the \emph{black-box} function $f_\V{s}(\cdot)$ can be very complex to implement using reversible quantum gates---for an $n$-bit hidden string, the number of simple gates needed to implement $f_\V{s}(\cdot)$ scales typically as $\mathcal{O}(4^n)$. Since the black box is a step in the algorithm, its serial execution time could in the worst-case even scale exponentially as $\mathcal{O}(4^n)$. The real breakthrough of this quantum algorithm lies in speeding up the query complexity and not the execution time per~se.

\subsection{Algorithm description}
Let us explore the BV algorithm in more detail. The $n$-qubit Hadamard operator is defined as:
\begin{equation}
H^{\otimes n} = \frac{1}{\sqrt{2^n}}\sum_{\V{x},\V{y} \in \{0,1\}^n} \left(-1\right)^{\braket{\V{x},\V{y}}}\ket{\V{y}}\bra{\V{x}}
\end{equation}
Given a specified Boolean function $f(\cdot)$, let us introduce an $(n+1)$-qubit black-box operator:
\begin{equation}
    U_{f(\cdot)} = \sum_{\V{x} \in \{0,1\}^n, y \in \{0,1\}} \ket{\V{x}}\bra{\V{x}} \otimes \ket{y \oplus f\left(\V{x}\right)}\bra{y}
\end{equation}
where we used $\oplus$ to denote Boolean (mod $2$) addition; and $\otimes$ to represent Kronecker product.
A nice property of this black-box operator is called \emph{phase kickback}: when we give a particular type of input to this operator, the hidden function $f(\cdot)$ appears in the phase of the output. Denoting $\ket{-} = {(\ket{0}-\ket{1})}/{\sqrt{2}}$, we get
\begin{equation}
    U_{f(\cdot)} \left(\ket{\V{x}}\ket{-}\right) = \left(-1\right)^{f\left(\V{x}\right)}\ket{\V{x}}\ket{-}
\end{equation}

For the BV algorithm, the Boolean function $f(\cdot)$ is just the dot product, $\braket{\V{s}, \V{x}}$, where \V{s} is a hidden string which we want to identify using the least number of queries. So,
\begin{equation}
U_{\V{s}} = \sum_{\V{x} \in \{0,1\}^n, y \in \{0,1\}} \ket{\V{x}}\bra{\V{x}} \otimes \ket{y \oplus \braket{\V{s}, \V{x}}}\bra{y}
\end{equation}

The entire BV algorithm is represented in Figure~\ref{BV:Fig:Block}. Analyzing the diagram, we see:
\begin{eqnarray}
    \ket{0}^n\ket{1} & \xrightarrow{H^{\otimes(n+1)}} & \frac{1}{\sqrt{2^n}} \sum_{\V{x}=0}^{2^n-1} \ket{\V{x}} \otimes \frac{\ket{0}-\ket{1}}{\sqrt{2}}
                     \quad \xrightarrow{U_s} \quad \frac{1}{\sqrt{2^n}} \sum_{\V{x}=0}^{2^n-1} \left(-1\right)^{\braket{\V{s}, \V{x}}}\ket{\V{x}} \otimes \frac{\ket{0}-\ket{1}}{\sqrt{2}} \nonumber\\
                     & \xrightarrow{H^{\otimes n}} & \frac{1}{\sqrt{2^n}} \sum_{\V{x},\V{y}=0}^{2^n-1} \left(-1\right)^{\braket{\V{s}, \V{x}} \oplus \braket{\V{x}, \V{y}}} \ket{\V{y}} \otimes \frac{\ket{0}-\ket{1}}{\sqrt{2}}
                     \quad \equiv \quad \ket{\V{s}} \otimes \frac{\ket{0}-\ket{1}}{\sqrt{2}}
\end{eqnarray}

\begin{figure}[!t]
    \centering
\includegraphics[width=0.90\textwidth]{BVBlockFig.png}
    \caption{Bernstein-Vazirani hidden string discovery quantum algorithm. The hidden string \V{s} is discovered with just a single query. The measurement result $\widetilde{\V{s}}$ gives estimated hidden string.\label{BV:Fig:Block}}
\end{figure}

\vspace*{-3ex}
\subsection{Algorithm implemented on IBM's $5$-qubit and $16$-qubit computers}
From the BV algorithm description in the previous section, we see that in any practical implementation of this algorithm, the main ingredient is the construction of the black-box oracle $U_{\V{s}}$ given a binary hidden string \V{s}. Let us see how this is done using an example length $2$ binary hidden string ``$01$''.  Equation~(\ref{BV:Tab:Perm}) below shows how the $3$-qubit operator maps the $2^3 = 8$ basis vectors.  The first line is the input binary vector (in the order $y, x_1, x_0$), and the second line is the output binary vector.
\begin{equation}
    U_{01} = \begin{pmatrix}
        000 & 001 & 010 & 011 & 100 & 101 & 110 & 111 \\
        000 & 101 & 010 & 111 & 100 & 001 & 110 & 011
    \end{pmatrix}
    \label{BV:Tab:Perm}
\end{equation}
This mapping is a permutation operator $U_{01} : \ket{\V{x}, y} \mapsto \ket{\V{x}, \braket{01, \V{x}} \oplus y}$; which is a special case of a unitary operator, as its matrix representation is unitary. The next task in implementation is to lower the unitary matrix operator $U_{01}$ to primitive gates available in the quantum computer's architecture. For the IBM-QX architecture, there are just three primitive hardware gates: ${\tt cx, u_1(), u_2(), u_3()}$. Here {\tt cx} is a control-not, where only certain control, target qubit pairs are allowed by the machine's connection topology graph. With,
\begin{equation}
    {\tt u}(\theta, \phi, \lambda) = \begin{pmatrix}
    e^{-i(\phi+\lambda)/2}\cos{\theta/2} & -e^{-i(\phi-\lambda)/2}\sin{\theta/2} \\
    e^{i(\phi-\lambda)/2}\sin{\theta/2} & e^{i(\phi+\lambda)/2}\cos{\theta/2}
\end{pmatrix},
\end{equation}
the available primitive gates ${\tt u_1,u_2,u_3}$ can be defined as,
$
{\tt u_1(\lambda)} = {\tt u}(0, 0, \lambda), \, {\tt u_2(\phi, \lambda)} = {\tt u}(\pi/2, \phi, \lambda), \, {\tt u_3(\theta, \phi, \lambda)} = {\tt u}(\theta, \phi, \lambda)
$. These have approximate time costs of ${\tt cx}: 1001, {\tt u_1}: 7, {\tt u_2}: 104, {\tt u_3}: 201$ (ns) respectively on a typical existing IBM-QX architecture---the timing model used is taken from IBM's published calibration models~\cite{IBM:QX:Models} for the primitive hardware gates.

In order to lower arbitrary unitary-matrices to the primitive gates listed above, we need to first perform a unitary diagonalization of the $2^{(n+1)} \times 2^{(n+1)}$ operator-matrix using multi-qubit-controlled single-qubit unitary Given's rotation operations. Such multi-qubit-controlled single-qubit operations can be lowered using standard techniques~\cite{NC:2010} to the hardware primitive gates ${\tt cx, u_1(), u_2(), u_3()}$. Even after this step we will be left with arbitrary ${\tt cx}$ gates. Since both {\tt ibmqx4, ibmqx5} computers have restricted {\tt cx} connectivity between qubits, we will need to first bring the control qubit ($c$) close to the target qubit ($t$) in the given topology (say swap qubit $c$ to position $c'$), by potentially doing upto $(m-2)$ pair-wise qubit-swaps on an $m$-qubit computer. Then if there is a directed edge $c' \rightarrow t$, we can apply ${\tt cx(} c',t{\tt)}$ gate directly. On the other hand, if there is an inverted directed edge $t \rightarrow c'$ on the machine topology, then we can reverse the roles of $c', t$ by applying $H^{\otimes 2}$ operators before and after ${\tt cx(} t,c'{\tt)}$. As the overall primitive gate counts scale as $\mathcal{O}(4^n)$ for arbitrary $n$-qubit unitary operators, the task quickly becomes hard to do by hand. We therefore wrote a piece of software called \emph{Quantum Netlist Compiler (QNC)}~\cite{NS:QNC2017} for performing this complex task. QNC can do much more than convert arbitrary unitary operators to OpenQASM-2.0 circuits---it has specialized routines implemented to generate circuits to do state-preparations, permutation operators, Gray coding to reduce gate counts, mapping to physical machine-topologies, as wells as gate-merging optimizations. Applying QNC tool to the unitary matrix $U_{\V{s}}$ gives us a corresponding quantum gate circuit $G_{\V{s}}$ as shown in Figure~\ref{BV:Fig:Block} for a specific bit-string \V{s}.

QNC generated black-box circuits with following gate-counts for the non-trivial $2$-bit hidden-strings: ``01'': $36$, ``11'': $38$, ``10'': $37$, with estimated execution time for critical path ${\sim}17\mu s$ on an ideal machine with all-to-all connection topology. For the $5$-qubit {\tt ibmqx4} machine the corresponding gate-counts where: ``01'': $42$, ``11'': $43$, ``10'': $41$, with estimated execution time for critical path ${\sim}15\mu s$, and for the $16$-qubit {\tt ibmqx5}, they were: ``01'': $66$, ``11'': $67$, ``10'': $67$, with estimated execution time for critical path ${\sim}28\mu s$. In all these cases, QNC used a specialized decomposition of $U_{01}$, considering its permutation matrix nature, and therefore was able to reduce gate-counts by $5\times$ over the case when this special structure was ignored. Considering that the machines' observed coherence times are of the order of ${\sim}60 \mu s$, these QNC optimizations were crucial to the feasibility of the resulting score.
The quantum score generated by QNC for $U_{01}$ for {\tt ibmqx4} is shown in Figure~\ref{BV:Fig:Score}. A similarly prepared score for $3$-bit hidden-string ``111'' had a gate-count of $428$ in the {\tt ibmqx4} architecture with an estimated execution time of $153 \mu s$ which was well above the machines' coherence times.
\begin{figure}[!hb]
    \centering
\includegraphics[width=0.98\textwidth]{visualIBMQASM.png}
    \caption{Quantum score for BV algorithm with hidden string ``01'' targeting the {\tt ibmqx4} architecture. There are $48$ primitive gates in this score, with critical path time ${\sim}16\mu s$.\label{BV:Fig:Score}}
\end{figure}

We tested the QNC generated quantum scores for all non-trivial $1$-qubit, $2$-bit and $3$-bit strings using the IBM-QISKit based local simulator. In all cases, the simulator produced the exact hidden-string as the measurement result, $100\%$ of the trials. We then tested all $1$-bit and $2$-bit strings on both the $5$-qubit {\tt ibmqx4} and the $16$-qubit {\tt ibmqx5} machines. The results are shown in Figure~\ref{BV:Fig:Results}. For $2$-bit strings, the worst case noise was observed for the string ``01'' on {\tt ibmqx4} when the qubits $q_0, q_1, q_2$ where used for $x_0, x_1, y$ respectively. Since the estimated critical path times exceeded the machines' coherence times for $3$-bit strings, we did not run those scores on the physical machines. Even for $2$-bit strings, the scores were quite long, and the results were quite noisy even with $8192$ machine-shots.
\begin{figure}[!hb]
    \centering
\includegraphics[width=0.26\textwidth]{BV01-ibmqx4.png}
    \hspace*{2ex}
\includegraphics[width=0.26\textwidth]{BV10-ibmqx4.png}
    \hspace*{2ex}
\includegraphics[width=0.26\textwidth]{BV11-ibmqx4.png}
    \caption{Results from running the BV algorithm for $8192$ shots on $2$-bit hidden-strings ``01'', ``10'' and ``11'' respectively (left to right) on {\tt ibmqx4}. Results for runs on {\tt ibmqx5} were similar, but more noisy due to longer scores.\label{BV:Fig:Results}}
\end{figure}

\subsection{Conclusion}
To conclude, we studied the academically important Bernstein-Vazirani quantum algorithm for hidden-string discovery. We then implemented a Quantum Netlist Compiler (QNC) to generate the black-box quantum circuits for specific IBM quantum machine topologies. We then executed the resulting scores on the simulator, as well as the $5$-qubit {\tt ibmqx4} and $16$-qubit {\tt ibmqx5} physical machines. In all cases tested, the hidden-string was identifiable from the dominant measured state provided enough number of experiments were performed. However, we also clearly observed decoherence, bias and noise issues in the physical machine results, and these issues were more pronounced as the critical path gate-count increased. As the number of primitive gates scales exponentially as the number of qubits for general unitary operators, we conclude that for successful implementation of most practical quantum algorithms, physical machines need to have large coherence times---so much so that larger coherence times are perhaps more important to have than more physical machine qubits.




==> Grover_Omalley/omalled_grover.tex <==

\section{Grover's Algorithm}

\subsection{Problem definition and background}
Grover's algorithm as initially described~\cite{grover} enables one to find (with probability $>1/2$) a specific item within a randomly ordered database of $N$ items using $O(\sqrt{N})$ operations.
By contrast, a classical computer would require $O(N)$ operations to achieve this.
Therefore, Grover's algorithm provides a quadratic speedup over an optimal classical algorithm.
It has also been shown~\cite{bennett1997strengths} that Grover's algorithm is optimal in the sense that no quantum Turing machine can do this in less than $O(\sqrt{N})$ operations.

While Grover's algorithm is commonly thought of as being useful for searching a database, the basic ideas that comprise this algorithm are applicable in a much broader context.
This approach can be used to accelerate search algorithms where a ``quantum oracle'' can be constructed that distinguishes the needle from the haystack.
The needle and hay need not be part of a database.
For example, it could be used to search to two integers $1<a<b$ such that $ab=n$ for some number $n$, resulting in a factoring algorithm
Of course, the performance of Grover's algorithm would not match the performance of Shor's algorithm~\cite{shor1994algorithms,shor1999polynomial} for this purpose.

Implementing the quantum oracle can be reduced to constructing a quantum circuit that flips an ancillary qubit, $q$, if a function, $f(\mathbf{x})$, evaluates to 1 for an input $\mathbf{x}$.
The function $f(\mathbf{x})$ is defined by
\begin{equation}\label{eq:grov_f}
	f(\mathbf{x})=
	\begin{cases}	
		1 & \text{if}~\mathbf{x}=\mathbf{x}^*\\
		0 & \text{if}~\mathbf{x}\ne\mathbf{x}^*
	\end{cases}
\end{equation}
where $\mathbf{x}=x_1x_2 \ldots x_n$ are binary strings and $\mathbf{x}^*$ is the specific string  that is being sought.
It may seem paradoxical at first that an algorithm for finding $\mathbf{x}^*$ is needed if such a function can be constructed.
The key here is that $f(\mathbf{x})$ need only recognize $\mathbf{x}^*$ -- it is similar to the difference between writing down an equation and solving an equation.
For example, it is easy to check if the product of $a$ and $b$ is equal to $n$, but harder to factor $n$.

Here we implement a simple instance of Grover's algorithm.
That is, the quantum oracle we utilize is a very simple one.
Let $\mathbf{x}= x_1x_2$ and we wish to find $\mathbf{x}^*$ such that $x^*_1=1$ and $x^*_2=1$.
While finding such an $x^*$ is trivial, we don a veil of ignorance and proceed as if it were not.
This essentially means that our function $f(\mathbf{x})$ is an AND gate. But the AND gate is not reversible and cannot be a quantum gate.
However, the Toffoli gate is similar to a classical AND gate, but comes with an extra feature that is useful for our purposes.
The Toffoli gate takes three bits as input and outputs three bits.
The first two bits are unmodified.
The third bit is flipped if the first two bits are 1. The unitary matrix correspondung to the Toffoli gate can be found in [REFERENCE TABLE]
In other words, the Toffoli gate implements our desired quantum oracle where the first two inputs are $x_1$ and $x_2$ and the third bit is the ancillary bit, $q$.
The behavior of the oracle in general is $\ket{\mathbf{x}}\ket{q}\rightarrow\ket{\mathbf{x}}\ket{f(\mathbf{x})\bigoplus q}$.

(About multi target search)

\subsection{Algorithm description}
Here we present a brief introduction to Grover's algorithm.
A more detailed account can be found in Nielsen and Chuang~\cite{Nielsen}. Let $N$ be the number of items (represented as bit strings) amongst which we are performing the search. This number will also be equal to the dimension the vector space we are working with. 
An operator, called the Grover operator, is they key piece of machinery in Grover's algorithm.
This operator is defined by
\begin{equation}
	G=(2\ket{\psi}\bra{\psi} - I)O
\end{equation}
where $\ket{\psi} =  \frac{1}{\sqrt{N}} \sum_i \ket{i} $ is the uniform superposition of all states and $O$ is the oracle operator (see Fig.~\ref{fig:abstractcircuit} for a concrete representation of this operator in the case where $\mathbf{x}$ consists of 2 bits).
The action of $(2\ket{\psi}\bra{\psi} - I)$ on an arbitrary state is
\begin{equation}
	(2\ket{\psi}\bra{\psi} - I) \sum_{i} a_i \ket{i} = \sum_{i} \left( 2\left<a\right> - a_i \right)\ket{i}
	\label{eq:inversion}
\end{equation}
where $\left<a\right>=\frac{\sum_i a_i}{N}$ and the sums are over all possible states (the sum is finite).
From equation~\ref{eq:inversion} one can see that the amplitude of each state is flipped about the mean amplitude.

\begin{figure}
	\includegraphics[width=\textwidth]{schematic.jpg}
	\caption{A schematic diagram of Grover's algorithm is shown.
	Note that in this case, one application of the Grover operator is performed.
	This is all that is necessary when there are only two bits in $\mathbf{x}$, but the Grover operator should be applied repeatedly for larger problems.}
	\label{fig:abstractcircuit}
\end{figure}

In order to leverage the Grover operator to successfully perform a search, $\ket{\mathbf{x}}\ket{q}$ must be appropriately initialized.
The initialization is carried out by applying a Hadamard transform ($H^{\bigotimes n}$) on $\ket{\mathbf{x}}$ and applying a Pauli X transform followed by a Hadamard transform ($HX$) to $q$.
This leaves $\ket{\mathbf{x}}$ in the uniform superposition of all states, $\ket{\psi}$, and $\ket{q}$ in the state $\frac{\ket{0}-\ket{1}}{\sqrt{2}}$.
After performing these operations, the system is in the state $\ket{\psi}\frac{\ket{0}-\ket{1}}{\sqrt{2}}$.
Using equation~\ref{eq:inversion}, we can now understand how the Grover operator works.
The action of the oracle operator on $\ket{\mathbf{x}^*}\frac{\ket{0}-\ket{1}}{\sqrt{2}}$ reverses the amplitude of that state
\begin{equation}
	O\ket{\mathbf{x}^*}\frac{\ket{0}-\ket{1}}{\sqrt{2}}\rightarrow\ket{\mathbf{x}^*}\frac{\ket{f(\mathbf{x}^*)\bigoplus0}-\ket{f(\mathbf{x}^*)\bigoplus1})}{\sqrt{2}} = \ket{\mathbf{x}^*}\frac{\ket{1}-\ket{0}}{\sqrt{2}} = -\ket{\mathbf{x}^*}\frac{\ket{0}-\ket{1}}{\sqrt{2}}
\end{equation}
A similar argument shows that all other states are unmodified by the oracle operator.
Combining this with equation~\ref{eq:inversion} reveals why the Grover operator is able to successfully perform a search.
Consider what happens on the first iteration:
The oracle operator makes it so that the amplitude of $\ket{\mathbf{x}^*}$ is below $\left< a \right>$ (using the notation of equation~\ref{eq:inversion}) while all the other states have an amplitude that is slightly above $\left<a\right>$.
The effect of applying $2\ket{\psi}\bra{\psi} - I$ is then to make $\ket{\mathbf{x}^*}$ have an amplitude above the mean while all other states have an amplitude below the mean.
The desired behavior of the Grover operator is to increase the amplitude of $\ket{\mathbf{x}^*}$ while decreasing the amplitude of the other states.
If the Grover operator is applied too many times, this will eventually stop happening.
The Grover operator should be applied exactly $\left\lceil\frac{\pi \sqrt{N}}{4}\right\rceil$ times after which a measurement will reveal $\mathbf{x^*}$ with probability close to $1$. 
In the case where $\mathbf{x}$ has two bits, a single application of Grover's operator is sufficient to find $\mathbf{x}^*$ with certainty (in theory).

\begin{algorithm}[H]
\caption{Grover's algorithm}
\begin{algorithmic} \label{alg:1}
    \STATE \textbf{Input:}
    \bindent
        \STATE $\bullet$ An Oracle operator effecting the transformation $\ket{x}\ket{q} \rightarrow  \ket{x}\ket{q \oplus f(x)}$.
    \eindent
    \STATE \textbf{Output:}
    \bindent
        \STATE $\bullet$ The unique bit string $\mathbf{x^*}$ satisfying Eq. \eqref{eq:grov_f}
    \eindent
    \STATE \textbf{Procedure:}
    \bindent
        \STATE \textbf{Step 1.} %Define $g : \mathbb{Z}_q^k \rightarrow G$ by mapping $(x_1,~\ldots, x_k) \rightarrow g(x) = a_1^{x_1} \cdot \cdot \cdot a_k^{x_k}$.
        
        \STATE \textbf{Step 2.} %Compute a set $y_1,~\ldots, y_l \in \mathbb{Z}_q^k/K$ of generators for $\mathbb{Z}_q^k/K$.
        \STATE \textbf{Step 3.} %Output the set $\{ g(y_1),~\ldots, g(y_l) \}$.
    \eindent
\end{algorithmic}
\end{algorithm}

\subsection{Algorithm implemented on IBM's 5-qubit computer}
Fig.~\ref{fig:ibmcircuit} shows the circuit that was designed to fit the ibmqx4 quantum computer.
The circuit consists of state preparation (first two time slots), a Toffoli gate (the next 13 time slots), followed by the $2\ket{\psi}\bra{\psi} - I$ operator (7 time slots), and measurement (the final 2 time slots).
We use $q[0]$ (in the register notation from Fig.~\ref{fig:ibmcircuit}) as the ancillary bit, $q$, and $q[1]$ and $q[2]$ as $x_1$ and $x_2$.
Note that the quantum computer imposes constraints on the possible source and target of CNOT gates.
Some care must be taken to choose the appropriate qubits to represent each variable so that the necessary CNOT gates can be implemented.
It is possible to circumvent some of the limitations in the source and target of the CNOT gates (i.e., the source and target can be reversed), but this requires increasing the depth of the circuit.
Our initial implementation utilized a Toffoli gate that used such an approach, but the circuit was significantly deeper and the results were inferior to the results with the circuit in Fig.~\ref{fig:ibmcircuit}.

Using the simulator, this circuit produces the correct answer $\mathbf{x}=(1,1)$ every time.
We executed 1,024 shots using the ibmqx4 and $\mathbf{x}=(1,1)$ was obtained 662 times with $(0,0)$, $(0, 1)$, and $(1, 0)$ occurring 119, 101, and 142 times respectively.
This indicates that the probability of obtaining the correct answer is approximately 65\%.
The deviation between the simulator and the quantum computer is apparently due to the depth of the circuit combined with the approximate nature of the quantum computer.
We note that our first implementation of this algorithm which used a Toffoli gate with a depth of 23 (compared to a depth of 13 here) obtained the correct answer 48\% of the time.

\begin{figure}
	\includegraphics[width=\textwidth]{score.jpg}
	\caption{The circuit that was executed on IBM's 5-qubit quantum computer (ibmqx4 was used).
	The first two time slots correspond to the state preparation.
	The next 13 time slots implement a Toffoli gate.
	The next 7 time slots implement the $2\ket{\psi}\bra{\psi} - I$ operator, and the final two time slots are used for observing $x_1$ and $x_2$.}
	\label{fig:ibmcircuit}
\end{figure}

\subsection{Conclusion}
We designed a circuit that implements an instance of Grover's algorithm for an IBM 5-qubit quantum computer.
The outcome was successful in the sense that the quantum computer successfully completed the search with a probability that is appreciably greater than 50\%.
However, the 65\% success rate that was obtained is much lower than the 100\% that is obtained by the simulator.
Deeper and more complex oracles would likely produce less satisfactory results, and this is in line with our experience implementing the oracle with a deeper implementation of the Toffoli gate.




==> Shor_figures/shor.tex <==
\section{Shor's Algorithm for Integer Factorization}

\subsection{Problem definition and background}
%2/3 page

The integer factorization problem asks, given an integer $N$ as an input, to find integers $1<N_1,N_2<N$ such that $N=N_1N_2$. This problem is hardest when $N_1$ and $N_2$ are primes with roughly the same number of bits. If $n$ denotes the number of bits of $N$, no algorithm with polynomial in $n$ time complexity is known. The straightforward algorithm that tries all factors from 2 to $\sqrt{N}$ takes time polynomial in $N$, but exponential in $n$. The most efficient known algorithm has running time $O\left(\exp \left(\sqrt[3]{\frac{64}{9}n(\log n)^2}\right)\right)$~\cite{Pomerance96atale}. In  practice, integers with 1000 or more bits are impossible to factor using known algorithms and classical hardware. The difficulty of factoring big numbers is the basis for the security of the RSA cryptosystem~\cite{Rivest:1978:MOD:359340.359342}, one of the most widely used public-key cryptosystems.

One of the most celebrated results in quantum computing is the development of a quantum algorithm for factorization that works in time polynomial in $n$. This algorithm, due to Peter Shor and known as Shor's algorithm~\cite{shor1994algorithms}, runs in $O(n^3\log n)$ time and uses $O(n^2\log n\log\log n)$ gates. The first implementation of that algorithm on a quantum computer was reported in 2001, when the number 15 was factored~\cite{2001Natur.414..883V}. The largest integer factored by Shor's algorithm so far is 21~\cite{2012NaPho...6..773M}.

In this section we describe Shor's algorithm and its implementation on an IBM Q experience quantum computer with 5 qubits.

\subsection{Algorithm description}%1.5 p.
\paragraph{Reducing factorization to period finding}
One way to factor an integer is by using modular exponentiation. Specifically, let an odd integer $N=N_1N_2$ be given, where $1<N_1,N_2<N$. Pick any integer $k<N$ such that $\gcd(k,N)=1$, where $\gcd$ denotes the greatest common divisor. One can show that there exists an exponent $p>0$ such that $k^p \equiv 1 \pmod N$. Recall that, by definition, $x \equiv y \pmod m$ if and only if $m$ divides $x-y$. Assume that $p$ is the smallest such number. If we find such $p$ and $p$ is even, then, by the definition of the modulo operation, $N$ divides
\begin{equation*}
  k^p-1=(k^{p/2}-1)(k^{p/2}+1).
\end{equation*}
But since the difference between $n_1=k^{p/2}+1$ and $n_2=k^{p/2}-1$ is 2, $n_1$ and $n_2$ have no common factor greater than 2. Moreover, both numbers are nonzeros by the minimality of $p$. Since $N=N_1N_2$ was assumed to be odd, then $N_1$ is a factor of either $n_1$ or $n_2$. Assume $N_1$ is a factor of $n_1$. Since $N_1$ is also a factor of $N$, then $N_1$ divides both $n_1$ and $N$ and one can find $N_1$ by computing $\gcd (n_1,N)$.
Hence, if one can compute such $p$, one can find the factors of $N$.

In order to find $p$, consider the modular exponentiation sequence $A=a_0,a_1,\dots$, where $a_i=k^i \pmod N$. Each $a_i$ is a number from the finite set $\{0,\dots,N-1\}$, and hence there exists indices $q$ and $r$ such that $a_q=a_r$. If $q$ and $r$ are the smallest such indices, one can show that $q=0$ and $A$ is periodic with period $r$. For instance, for $N=15$ and $k=7$, the modular exponentiation sequence is $1,7,4,13,1,7,4,13,1,\dots$ with period 4. Since the period 4 is an even number, we can apply the above idea to find
\begin{equation*}
  7^4 \bmod 15 \equiv 1 \Rightarrow 7^4-1 \bmod 15 \equiv 0 \Rightarrow (7^2-1)(7^2+1) \bmod 15 \equiv 0 \bmod 15 \Rightarrow \mbox{15 divides } 48\cdot 50,
\end{equation*}
which can be used to compute the factors of 15 as $\gcd(48,15)=3$ and $\gcd(50,15)=5$.

Finding the period of the sequence $A$ is, however, not classically easier than directly searching for factors of $N$, since one may need to check as many as $\sqrt{N}$ different values of $A$ before encountering a repetition. However, with quantum computing, the period can be found in polynomial time using the Quantum Fourier Transform (QFT). In the next subsection we will give a definition and describe a circuit for computing QFT.

\paragraph{Quantum Fourier Transform}
The Discrete Fourier Transform (DFT) takes as an input a vector $X$ of size $N$ and outputs vector $Y=WX$ where the \textit{Fourier matrix} $W$ is defined by
\begin{equation*}
W=\frac{1}{\sqrt{N}}
\begin{bmatrix}
    1       & 1 & 1 & \dots & 1 \\
    1       & \omega & \omega^2 & \dots & \omega^{N-1} \\
    1       & \omega^2 & \omega^4 & \dots & \omega^{2(N-1)} \\
    \vdots & \vdots & \vdots & \ddots & \vdots &  \\
    1       & \omega^{N-1} & \omega^{2(N-1)} & \dots & \omega^{(N-1)(N-1)}
\end{bmatrix},
\end{equation*}
where the $ij$-the element of the matrix is $W_{ij}=\omega^{ij}$ and $\omega$ is a primitive $N$-th root of unity ($\omega^N=1$). A straightforward implementation of the matrix-vector multiplication takes $O(N^2)$ operations, but, by using the special structure of the matrix, the Fast Fourier Transform (FFT) does the multiplication in only $O(N\log N)$ time. The algorithm is recursive and is illustrated on Figure~\ref{fig:FFT}.
\begin{figure}[htbp]
\includegraphics{Figures/FFT2}
\caption{Fast Fourier Transform circuit, where $j$ denoted a row from the top half of the circuit and $\omega^j$ denotes that the corresponding value is multiplied by $\omega^j$. The plus and minus symbols indicate that the corresponding values have to be added or subtracted, respectively.}
\label{fig:FFT}
\end{figure}
The Quantum Fourier Transform (QFT) is defined as a transformation between two quantum states that are determined using the values of DFT (FFT)\@. If $W$ is a Fourier matrix and $X=\{x_i\}$ and $Y=\{y_i\}$ are vectors such that $Y=WX$, then QFT is defined as the transformation
\begin{equation*}
  {\cal QFT}(\sum_{k=0}^{N-1}x_k\ket{k})= \sum_{k=0}^{N-1}y_k\ket{k}.
\end{equation*}
The implementation of QFT mimics the stages (recursive calls) of FFT, but implements each stage using only $n+1$ additional gates per stage. A single Hadamard gate on the last (least significant) bit implements the additions/subtractions of the outputs from the recursive call and the multiplications by $\omega^j$ are done using $n$ controlled phase gates. The circuit for $n=5$ is shown on Figure~\ref{fig:QFT}.
\begin{figure}[htbp]
\includegraphics[scale=0.9]{Figures/QFT_5}
\caption{A Quantum Fourier Transform circuit for five qubits ($n=5$).}
\label{fig:QFT}
\end{figure}

The property of QFT that is essential for the factorization algorithm is that it can ``compute'' the period of a periodic input. Specifically, if the input vector $X$ is of length $M$ and period $r$, where $r$ divides $M$, and its elements are of the form
\begin{equation*}
x_i=\begin{cases}
\sqrt{r/M} & \text{if $i \bmod r \equiv s$} \\
0 & \text{otherwise}
\end{cases}
\end{equation*}
for some offset $s<r$, and ${\cal QFT}\left(\sum_{i=0}^Mx_i\ket{i}\right)=\sum_{i=0}^My_i\ket{i}$, then
\begin{equation*}
y_i=\begin{cases}
1/\sqrt{r} & \text{if $i \bmod M/r \equiv 0$} \\
0 & \text{otherwise}
\end{cases}
\end{equation*}
i.e.,~the output has nonzero values at multiples of $M/r$ (the values $\sqrt{r/M}$ and $1/\sqrt{r}$ are used for normalization). Then, in order to factor an integer, one can find the period of the corresponding  modular exponentiation sequence using QFT, if one is able to encode its period in the amplitudes of a quantum state (the input to QFT).

A period-finding circuit for solving the integer factorization problem is shown on Figure~\ref{fig:period}~\cite{Dasgupta:2006:ALG:1177299}.
%
\begin{figure}[htbp]
\includegraphics[scale=0.9]{Figures/period_finding2}
\caption{Illustration of the period-finding circuit, where $m=2n$ and $M=2^m$.}
\label{fig:period}
\end{figure}
The first QFT on register~$A$ produces an equal superposition of the qubits from $A$, i.e.,~the resulting state is
\begin{equation*}
  \frac{1}{\sqrt{M}}\sum_{i=0}^M\ket{i,0}.
\end{equation*}
Next is a modular exponentiation circuit that computes the function $f(i)=x^i \pmod N$ on the second register. The resulting state is
\begin{equation*}
  \frac{1}{\sqrt{M}}\sum_{i=0}^M\ket{i,f(i)}.
\end{equation*}
Before we apply the next QFT transform, we do a measurement of register~$B$. (By the principle of deferred measurement~\cite{Nielsen} and due to the fact that register~$A$ and~$B$ don't interact from that point on, we don't have to actually implement the measurement, but it will help to understand the final output.) If the value measured is $s$, then the resulting state becomes
\begin{equation*}
  \frac{1}{\sqrt{M/r}}\sum_{\substack{i=0\\f(i)=s}}^M\ket{i,s},
\end{equation*}
where $r$ is the period of $f(i)$.
In particular, register~$A$ is a superposition with equal non-zero amplitudes only of $\ket{i}$ for which $f(i)=s$, i.e.,~it is a periodic superposition with period $r$. Given the property of QFT, the result of the transformation is the state
\begin{equation*}
  \frac{1}{\sqrt{r}}\sum_{i=0}^r\ket{i(M/r),s}.
\end{equation*}
Hence, the measurement of register~$A$ will output a multiple of $M/r$. If the simplifying assumption that $r$ divides $M$ is not made, then the circuit is the same, but the classical postprocessing is a bit more involved.

\subsection{Algorithm implemented on IBM's 5-qubit computer}
We implemented the algorithm on ibmqx4, a 5-qubit quantum processor from the IBM Quantum Experience, in order to factor number 15 with $x=11$. The circuit as described on Figure~\ref{fig:period} requires 12 qubits and 196 gates, too large to be implemented on ibmqx4. Hence, we used an optimized/compiled version from~\cite{2001Natur.414..883V} that uses 5 qubit and 11 gates (Figure~\ref{fig:shor_circuit}).
\begin{figure}[htbp]
\includegraphics[scale=0.4]{Figures/shor_11_25}
\caption{Circuit for Shor's algorithm for $N=15$ and $x=11$.}
\label{fig:shor_circuit}
\end{figure}
The results from the measurements are shown on Figure~\ref{Djidjev:fig:results}.
\begin{figure}[htbp]
\includegraphics[scale=0.6]{Figures/results_simulator.png}\hfill
\includegraphics[scale=0.6]{Figures/results_ibmqx4.png}
\caption{Output from the circuit from Figure~\ref{fig:shor_circuit} implemented on the simulator (left) and ibmqx4 (right).}
\label{Djidjev:fig:results}
\end{figure}

The periods found by the simulator are $p=0$, which is ignored as a trivial period, and $p=4$, which is a good one. Since $M=8$, we can conclude that $r$ divides $M/p=8/4=2$, hence $r=2$. Then $15$ divides
\begin{equation*}
  (x^r-1)=(11^2-1)=(11-1)(11+1)=10 \cdot 12.
\end{equation*}
By computing $\gcd(15,10)=5$ and  $\gcd(15,12)=3$, we find the factors of 15.

The output from ibmqx4 finds the same periods 0 and 4 with the highest probabilities, but contains much more noise.


\subsection{Conclusion}
Shor's quantum factorization algorithm reduces to finding the period of a periodic sequence, and such period can be found using Quantum Fourier Transform. Unless optimized, the general-case circuit for Shor's algorithm for factorization of the number 15 is too large, both with respect to the number of qubits as well as the number of gates, to be implemented on a 5-qubit processor. We were able to implement a compiled optimized version that produced correct results, however, comparing the results produced by the simulator and the real quantum processor showed the considerable noise of the latter.

